A maximum-entropy approach to off-policy evaluation in average-reward MDPs

This work focuses on off-policy evaluation (OPE) with function approximation in infinite-horizon undiscounted Markov decision processes (MDPs). For MDPs that are ergodic and linear (i.e. where rewards and dynamics are linear in some known features), we provide the first finite-sample OPE error bound, extending existing results beyond the episodic and discounted cases. In a more general setting, when the feature dynamics are approximately linear and for arbitrary rewards, we propose a new approach for estimating stationary distributions with function approximation. We formulate this problem as finding the maximum-entropy distribution subject to matching feature expectations under empirical dynamics. We show that this results in an exponential-family distribution whose sufficient statistics are the features, paralleling maximum-entropy approaches in supervised learning. We demonstrate the effectiveness of the proposed OPE approaches in multiple environments.

==> kernelization.tex <==
\section{Kernelization}
\label{app:kernelization}

In this section, we show a simple way to kernelize our distribution using kernel ridge regression for the model. 
Consider maximizing the entropy of the joint state-action distribution $d_\pi(s, a)$ rather than just the marginal, subject to matching feature statistics:
\begin{align}
\min_{d \in \Delta_{\cS}} & \; \sum_{s, a} d(s, a) \ln d(s, a) 
\quad
{\rm s.t.}  \; 
   \sum_{s, a} d(s, a) \overline \phi(s, a)^\top W_\pi=  \sum_{s, a} d(s, a) \phi(s, a)^\top \,,
\end{align}
where 
$\overline \phi = \left[ \begin{smallmatrix}  \phi \\ 1  \end{smallmatrix}\right]$ and 
$W_\pi = \left[ \begin{smallmatrix} M_\pi  \\ b_\pi^\top  \end{smallmatrix}\right]$.
The optimal solution is in the exponential family and of the form 
\begin{align*}
    d_\pi(s, a) &= \exp( (\phi(s, a)^\top  - \overline \phi(s, a)^\top W_\pi )\theta_\pi - F(\theta_\pi |W_\pi)).
\end{align*}
The parameters $\theta_\pi$ correspond to the minimizer of the dual problem,
\[
\theta_\pi = \argmin_\theta D(\theta) := F(\theta | W_\pi) \;.
\]

% The dual gradient w.r.t. 
% $\overline \theta$ is
% \begin{align}
%      \nabla_\theta D( \overline \theta) = \sum_{s, a} d_\pi(s, a) (I - W_\pi)^\top \overline \phi(s, a)
    % \quad {\rm where} \; \rho(s, a) = \frac{d_\pi(s, a | \theta_\pi, M_\pi)}{d_\beta(s, a | \theta_\beta, M_\beta)}
% \end{align}
Let $\Phi$ be the $T \times (m +1)$ matrix of state-action feature vectors $\overline \phi(s, a)$, let $K = \Phi \Phi^\top$, and let $\Psi$ be the $T \times m$ matrix of next-state expected features $\phi(s', \pi)$. 
We estimate $W_\pi$ as:
\begin{align*}
    \widehat W_\pi &= (\Phi^\top \Phi + b I)^{-1}\Phi^\top \Psi = \Phi^\top (K + bI)^{-1} \Psi
\end{align*}
Let $z = (s, a)$ and let $k(z, z')$ be a kernel function on a reproducing kernel Hilbert space. Let ${\bf k}_z = \sum_{t=1}^T k(z, z_t)$. We can write the joint distribution estimate as
\begin{align*}
    \hat d_\pi(s, a) & \propto \exp( \phi(s, a)^\top \theta_\pi - \overline \phi(s, a)^\top \widehat W_\pi  \theta_\pi) \\
    &= \exp(  \phi(s, a)^\top \theta_\pi  - {\bf k}_z^\top (K + bI)^{-1}\Psi \theta_\pi )\,.
\end{align*}
The above formulation allows us to use kernel ridge regression in place of linear regression for the feature model. The parameters $\theta_\pi$ can be estimated using gradient descent as before, where the gradient can be computed as:
\begin{align*}
    \nabla_\theta D(\theta ) = \sum_{(s, a) \sim d_\beta} \frac{d_\pi(s, a | \theta)}{d_\beta(s, a)} (\phi(s, a) - \Psi^\top (K + bI)^{-1} {\bf k}_z) \,.
\end{align*}
% To get away from features entirely, we can consider $\phi(s, a)$ to be an indicator for each example in the data. 


\iffalse
{\bf Breaking the curse of the horizon} \citep{liu2018breaking}. 
\nevena{longer description for now}
Let $\rho(s) = \frac{\mu_\pi(s)}{\mu_\beta(s)}$ be the stationary distribution ratio, and let $\Delta(\rho; s, a, s') = \rho(s)\pi(a|s) / \beta(a|s) - \rho(s')$. The true $\rho$ satisfies $E_{\mathcal{D}_\beta}[\Delta(\rho; s, a, s')] = 0$, but this expectation is difficult to estimate directly as we need multiple $(s, a)$ pairs transitioning to the same $s'$. \citet{liu2018breaking} note that we can instead require $L(\rho, \phi) = \E[\Delta(\rho; s, a, s;) \phi(s')] = 0$ for all functions $\phi(\cdot)$. This motivates the minimax problem, where $z_\rho = \sum_{s}\rho(s)$:
\begin{align*}
    \min_\rho D(\rho) := \max_{\phi \in \cF} L(\rho / z_\rho, \phi)^2 \,.
\end{align*}
When $\cF$ is a unit ball in a reproducing kernel Hilbert space with a positive definite kernel $k(s, \overline s)$, the maximization can be done in closed form as
\begin{align*}
    D(\rho) := \E_{\cD_\beta} [\Delta(w; s, a, s') \Delta(w; \overline s, \overline a, \overline s')k(s', \overline s')]
\end{align*}
\fi

==> kernelization_m.tex <==
\section{Kernelization}

Given a trajectory $\{(s_t, a_t, r_t)\}_{t=1}^{T+1}$,
let $\overline  \Phi$ and $\Phi$ be the $T\times (m+1)$ and $T\times m$  matrices of the extended ($ \overline  \phi(s_t, a_t)$ ) and regular ($\phi(s_t, a_t)$) feature vectors, respectively. Also let $\Psi$ be a $T \times m$ matrix of corresponding next-state regular feature vectors $  \phi(s_{t+1}, \pi)$.

Let's try to compute $\nabla_\theta F(\theta | M_\pi) = \E_{\mu_\pi}[ (I - M_\pi^\top) \phi(s, \pi)]$
\begin{align*}
\E_{\mu_\pi}[ (I - M_\pi^\top) \phi(s, \pi)] & = 
\sum_{s} (I - M_\pi^\top) \phi(s, \pi) \mu_\pi(s) 
= \sum_{s} (I - M_\pi^\top) \mu_\pi(s)  \sum_a \phi(s, a) \pi(a|s) \\
& = \sum_{s,a} (I - M_\pi^\top) \phi(s, a) \mu_\pi(s) \pi(s,a) = \sum_{s,a} (I - M_\pi^\top) \phi(s, a) \mu_\pi(s,a)
\end{align*}
The off-policy estimate of the gradient is therefore:
\begin{align*}
\E_{\mu_\pi}[ (I - M_\pi^\top) \phi(s, \pi)] & = \sum_{s,a \in \mathcal{D}_\beta} (I - M_\pi^\top) \phi(s, a) \frac{\mu_\pi(s) \pi(a|s)}{\mu_\beta(s) \beta(a|s)}
\end{align*}
given that our data is generated by policy $\beta$.
We first find a sample average estimate of $E_{\mu_\beta}[(I - M_\pi^\top) \phi(s, a) \mu_\pi(s)]$. \nevena{Let $\hat \mu_\pi$ be a length-$T$ vector whose $t^{th}$ entry corresponds to $\hat \mu(s_t)$ - right?} \mehrdad{True.}
\nevena{Also should we have $\Psi$ below instead of $\Phi$? There is a way to use $\Phi$ below instead, I can write it} \mehrdad{Please write it. Having $\Psi$ makes the subsequent steps even easier. But, in the above derivation $\phi(s,a)$ is involved not $\phi(s,\pi)$. The policy $\pi$ is absorbed into the importance ratios.... (everything is getting more and more confusing (and interesting of course!)) } \nevena{I see, that's exactly what I had in mind too, but in that case I think you need $\hat d = \hat \mu \otimes \pi $ below and not $\hat \mu$. Actually we need the importance ratio $\hat d_\pi / \hat d_\beta$? }
\mehrdad{True. I see. So

[Option 1]: Just multiply the estimation with $\frac{\pi(a|s)}{\beta(a|s)}$. These two values are given and won't change anything. For example, I define a diagonal $T \times T$ matrix $D_\pi$ with $\pi(a_t |s_t)$ in the diagonals and replace  $\hat \mu_\pi$  with $D_\pi \hat \mu_\pi$ in the followings.
}
\nevena{Yes that works} \mehrdad{But we still to take care of the other issue you mentioned in the next paragraph. hum?}


\mehrdad{[Option 2]:}
\begin{align}
\nabla_\theta \Bigl( F(\theta | \widehat  M_\pi) -\hat b_\pi^\top \theta \Bigr)
& =(I-\widehat M_\pi^\top)  \Phi^\top \hat \mu_\pi  - \hat b_\pi
=  \Phi^\top \hat \mu_\pi -  [ \widehat M_\pi^\top \quad \hat b_\pi] \begin{bmatrix}   \Phi^\top \hat \mu_\pi  \vspace{3pt} \\ 1 \end{bmatrix} \\
& =  (\Phi^\top  -  [ \widehat M_\pi^\top \quad \hat b_\pi] \,   \overline \Phi^\top) \hat \mu_\pi 
\end{align}
Moreover, according to Equation~\eqref{eq:m_estimation} and utilizing matrix inversion identity one can write
\begin{equation}
\begin{bmatrix} \widehat M_\pi \vspace{3pt} \\ \hat b_\pi^\top \end{bmatrix}
= (\overline \Phi^\top \overline \Phi + \Lambda)^{-1} \overline \Phi^\top   \Psi 
= \overline \Phi^\top (\overline \Phi \overline \Phi^\top  + \Lambda)^{-1}    \Psi,
\end{equation}
And, according to Equation~\eqref{eq:exp_family_form} we have
\begin{equation}
\ln \hat \mu_\pi \propto   \Phi (I-\widehat M_\pi)  \theta
=    \Phi (I-[\overline \Phi^\top (\overline \Phi \overline \Phi^\top  + \Lambda)^{-1}   \Psi]_+)  \theta
= \Phi \theta -\Phi  \Phi^\top (\overline \Phi \overline \Phi^\top  + \Lambda)^{-1}    \Psi \theta.
\end{equation}
where the $[A]_+$ means that the matrix $A$ with the last row dropped.

Combining the above two derivations we get:
\nevena{But below you are using $\ln \mu$ instead of $\mu$? Maybe we can just assume $\mu$ is a pre-computed vector? (computed as you worked out above)} \mehrdad{Yep. We can just put an $\exp$ before. The kernelization for $\mu$ doesn't involve the preceding term. They look independent. Right? Also $\hat \mu$ should sum to 1? Then, the normalizer can be absorbed into learning rate.}
\nevena{Yeah I just say that we normalize empirically in the main text. The identity matrix in $I - M_\pi$ and $b_\pi$ make kernelization difficult it seems :/ }
\mehrdad{look at the paper I sent in the slack. I think, they have the same issue. But solved it via the representation trick.}
\begin{align}
\nabla_\theta \Bigl( F(\theta | \widehat  M_\pi) -\hat b_\pi^\top \theta \Bigr)
 =  & (\Phi^\top  -  \Psi^\top  (\overline \Phi \overline \Phi^\top  + \Lambda^\top)^{-1} \overline \Phi \overline \Phi^\top)  
{\color{blue} \exp}(  \Phi \theta -\Phi  \Phi^\top (\overline \Phi \overline \Phi^\top  +  \Lambda)^{-1}    \Psi \theta) \\  =   &
\Phi^\top (  \Phi \theta -\Phi  \Phi^\top (\overline \Phi \overline \Phi^\top  +  \Lambda)^{-1}    \Psi \theta) - \\ &
 \Psi^\top  (\overline \Phi \overline \Phi^\top  + \Lambda^\top)^{-1} \overline \Phi \overline \Phi^\top
(  \Phi \theta -\Phi  \Phi^\top (\overline \Phi \overline \Phi^\top  +  \Lambda)^{-1}    \Psi \theta)
\end{align}
Note that $\Phi$ and $\Psi$ can be seen as submatrices of a $(T+1)\times m$ matrix $\Omega$ that includes all the $T+1$ features observed.  $\Phi$ is the upper $T \times m$ submatrix and $\Psi$ is shifted by one row, ie, the lower $T \times m$ submatrix. 
\nevena{hm, but $\Psi$ also includes an expectation w.r.t $\pi$?} \mehrdad{emmm. This has always been confusing for me. My latest thought is that the shifted observed pair can be seen as an unbiased sample from the expected (w.r.t. $\pi$) next feature pair. $E[\phi(s_{t+1}, a_{t+1})] = \sum_{s', a'} \pi(a' | s') P(s' | s_t, a_t) \phi(s', a')^\top$}
\nevena{hey m! I don't think that's true because the data is generated by $\beta$. so the next shifted example is a sample from $\beta$, not $\pi$. But $\phi(s, pi)$ is just a linear combination of $\phi(s, a)$, i.e. $\phi(s, \pi) = \sum_a \pi(a|s) \phi(s, a)$, so it lies in the same feature space. it is confusing...}
\mehrdad{Yep. It's involving another policy. It would have been good to work with just observed ones. But, how?
The linear combination may make things complicatd. Because then per observed state we have to consider all the actions. This means that our bases should include all $T \times |A|$ pairs. But still independent of $m$.}
The columns of $\Phi^\top$ and $\Psi^\top$ are subset of the columns of $\Omega^\top$. Therefore, the gradient update for $\theta$ lies in the space spanned by columns of $\Omega^\top$. We introduce dual variables $\zeta = [\zeta_1, \ldots, \zeta_{T+1}]^\top$. 
Then, $\theta = \sum_{i=1}^{T+1} \zeta_i  \phi(s_i, a_i)= \Omega^\top \zeta$ according to the representer theorem. 

Therefore, one can write the update equation in terms of  $ K = \Phi  \Phi^\top $, $\overline K =\overline \Phi \overline \Phi^\top = K + \mathbf{1}^\top \mathbf{1}$, $H=\Psi \Phi^\top $. Note also that  $ \Phi \theta =  \Phi \Omega^\top \zeta = K_1 \zeta $ and  $\Psi \theta_\pi = \Psi \Omega^\top \zeta = K_2 \zeta$. This way, we turned the problem that depended on features to a problem that is dependent to kernels. These are all submatrices of the kernel matrix.
\begin{align}
\nabla_\zeta =   &
 (  K_1 \zeta - K (\overline K  +  \Lambda)^{-1}   K_2 \zeta) -
  (\overline K  + \Lambda^\top)^{-1} \overline K
(   K_1 \zeta -K (\overline K  +  \Lambda)^{-1}     K_2 \zeta)
\end{align}

Similarly we can get an (on-policy) estimate of $\mu_\beta$.

\nevena{So how to get $\zeta$?}
-----------------------------------------------------------

Let $\overline  \Phi$ be a $T\times m$ matrix of feature vectors $ \overline  \phi(s_t, a_t)$ in the data episode, and let $\overline  \Psi$ be a $T \times m$ matrix of corresponding next-state feature vectors $\overline  \phi(s_{t+1}, \pi)$.
Following Equations ~\eqref{eq:theta_optization} and ~\eqref{eq:grad_f} our gradient based update rule can be written as
\begin{align}
\nabla_\theta \Bigl( F(\theta | \widehat  M_\pi) -\hat b_\pi^\top \theta \Bigr)
& = \frac{1}{T}(I-\widehat M_\pi^\top)  \Phi^\top \mathbf{1} - \hat b_\pi
= \frac{1}{T} \Phi^\top \mathbf{1} -  [ \widehat M_\pi^\top \quad \hat b_\pi] \begin{bmatrix} \frac{1}{T}  \Phi^\top \mathbf{1}  \vspace{3pt} \\ 1 \end{bmatrix} \\
& = \frac{1}{T} (\Phi^\top  -  [ \widehat M_\pi^\top \quad \hat b_\pi] \,   \overline \Phi^\top) \mathbf{1} 
\end{align}
Moreover, according to Equation~\eqref{eq:m_estimation} and utilizing matrix inversion identity one can write
\begin{equation}
\begin{bmatrix} \widehat M_\pi \vspace{3pt} \\ \hat b_\pi^\top \end{bmatrix}
= (\overline \Phi^\top \overline \Phi + \Lambda)^{-1} \overline \Phi^\top   \Psi 
= \overline \Phi^\top (\overline \Phi \overline \Phi^\top  + \Lambda)^{-1}    \Psi,
\end{equation}
Therefore,
\begin{align}
\nabla_\theta \Bigl( F(\theta | \widehat  M_\pi) -\hat b_\pi^\top \theta \Bigr)
& = \frac{1}{T} (\Phi^\top  -  \Psi^\top  (\overline \Phi \overline \Phi^\top  + \Lambda^\top)^{-1} \overline \Phi \overline \Phi^\top) \mathbf{1} 
\end{align}



----------------------------------------------------

Let's compute the ingredients separately:
\begin{equation}
\ln \hat \mu_\pi \propto  \overline \Phi (I-\widehat M_\pi)  \theta_\pi
=   \overline \Phi (I-\overline \Phi^\top (\overline \Phi \overline \Phi^\top  + b I)^{-1}   \overline \Psi)  \theta_\pi
= \overline \Phi \theta_\pi -\overline \Phi \overline \Phi^\top (\overline \Phi \overline \Phi^\top  + b I)^{-1}   \overline \Psi \theta_\pi.
\end{equation}
For $(I-\widehat M_\pi) \overline \Phi^\top $ first note that:
\begin{equation}
\widehat M_\pi 
= (\overline \Phi^\top \overline \Phi + b I)^{-1} \overline \Phi^\top  \overline \Psi 
= \overline \Phi^\top (\overline \Phi \overline \Phi^\top  + b I)^{-1}   \overline \Psi,
\end{equation}
thus,
\begin{equation}
(I-\widehat M_\pi) \overline \Phi^\top = \overline \Phi^\top (I-(\overline \Phi \overline \Phi^\top  + b I)^{-1} \overline \Psi \overline \Phi^\top )
\end{equation}
Therefore, 
\begin{equation}
\theta_\pi^{new} =  \theta_\pi + \nu
\overline \Phi^\top (I-(\overline \Phi \overline \Phi^\top  + b I)^{-1} \overline \Psi \overline \Phi^\top )
\exp(\overline \Phi \theta_\pi -\overline \Phi \overline \Phi^\top (\overline \Phi \overline \Phi^\top  + b I)^{-1}   \overline \Psi \theta_\pi)
\end{equation}
where, $\nu$ is the learning rate which has absorbed the constant normalizer of $\mu_\pi$ too.
The gradient update for $\theta_\pi$ lies in the space spanned by columns of $\overline \Phi^{\top}$. We introduce dual variables $\zeta = [\zeta_1, \ldots, \zeta_{T}]^\top$. Then, $\theta_\pi = \sum_{i=1}^{T} \zeta_i  \overline \Phi(s_i, a_i)=\overline \Phi^\top \zeta$ according to the representer theorem. 
Therefore, one can write the update equation in terms of $K =\overline \Phi \overline \Phi^\top $, $H=\overline \Psi \overline \Phi^\top $. Note also that  $\overline \Phi \theta_\pi = \overline \Phi \overline \Phi^\top \zeta = K \zeta $ and  $\overline \Psi \theta_\pi = \overline \Psi \overline \Phi^\top \zeta = H \zeta $. This way, we turned the problem that depended on features to a problem that is dependent to kernels:
\begin{equation}
\zeta^{new} =  \zeta + \nu
(I-(K  + b I)^{-1} H)
\exp(K\zeta - K(K  + b I)^{-1}  H\zeta)
\end{equation}
After finding the optimal $\zeta$ the distribution $\mu_\pi$ is computed accordingly:
\begin{equation}
\ln \mu_\pi \propto  \
K\zeta -K (K  + b I)^{-1} H \zeta.
\end{equation}
Similarly, we can compute $\mu_\beta$.

\mehrdad{The above is like a draft of the proof. I'll write a better version and update the notations to include $tilde$ and $hat$ wherever needed later.}


